Search for the critical point of strongly-interacting matter in ${}^{40}$Ar + ${}^{45}$Sc collisions at 150A GeV/c using scaled factorial moments of protons

The critical point of dense, strongly interacting matter is searched for at the CERN SPS in ${}^{40}$Ar + ${}^{45}$Sc collisions at 150A GeV/c. The dependence of second-order scaled factorial moments of proton multiplicity distribution on the number of subdivisions of transverse momentum space is measured. The intermittency analysis is performed using both transverse momentum and cumulative transverse momentum. For the first time, statistically independent data sets are used for each subdivision number. The obtained results do not indicate any statistically significant intermittency pattern. An upper limit on the fraction of critical proton pairs and the power of the correlation function is obtained based on a comparison with the Power-law Model developed for this purpose.

==> include/na61Acknowledgments.tex <==
We would like to thank the CERN EP, BE, HSE and EN Departments for the
strong support of NA61/SHINE.

This work was supported by
the Hungarian Scientific Research Fund (grant NKFIH 138136\slash138152),
the Polish Ministry of Science and Higher Education
(DIR\slash WK\slash\-2016\slash 2017\slash\-10-1, WUT ID-UB), the National Science Centre Poland (grants
2014\slash 14\slash E\slash ST2\slash 00018, %AR, settled
2016\slash 21\slash D\slash ST2\slash 01983, %MMP, settled
2017\slash 25\slash N\slash ST2\slash 02575, %AT, settled
2018\slash 29\slash N\slash ST2\slash 02595, %AM, completed, not settled
2018\slash 30\slash A\slash ST2\slash 00226, %MG, in progress
2018\slash 31\slash G\slash ST2\slash 03910, %SK, in progress
2019\slash 33\slash B\slash ST9\slash 03059, %DB, LT (astro), in progress
2020\slash 39\slash O\slash ST2\slash 00277), %MR, in progress
the Norwegian Financial Mechanism 2014--2021 (grant 2019\slash 34\slash H\slash ST2\slash 00585),
the Polish Minister of Education and Science (contract No. 2021\slash WK\slash 10),
the Russian Science Foundation (grant 17-72-20045),
the Russian Academy of Science and the
Russian Foundation for Basic Research (grants 08-02-00018, 09-02-00664 and 12-02-91503-CERN),
the Russian Foundation for Basic Research (RFBR) funding within the research project no. 18-02-40086,
the Ministry of Science and Higher Education of the Russian Federation, Project "Fundamental properties of elementary particles and cosmology" No 0723-2020-0041,
the European Union's Horizon 2020 research and innovation programme under grant agreement No. 871072,
the Ministry of Education, Culture, Sports,
Science and Tech\-no\-lo\-gy, Japan, Grant-in-Aid for Sci\-en\-ti\-fic
Research (grants 18071005, 19034011, 19740162, 20740160 and 20039012),
the German Research Foundation DFG (grants GA\,1480\slash8-1 and project 426579465),
%
the Bulgarian Ministry of Education and Science within the National
Roadmap for Research Infrastructures 2020--2027, contract No. D01-374/18.12.2020,
%
Ministry of Education
and Science of the Republic of Serbia (grant OI171002), Swiss
Nationalfonds Foundation (grant 200020\-117913/1), ETH Research Grant
TH-01\,07-3 and the Fermi National Accelerator Laboratory (Fermilab), a U.S. Department of Energy, Office of Science, HEP User Facility managed by Fermi Research Alliance, LLC (FRA), acting under Contract No. DE-AC02-07CH11359 and the IN2P3-CNRS (France).\\

The data used in this paper were collected before February 2022.


==> include/na61Authors.tex <==
% based on XML DB with time Fri Apr 28 12:49:46 2023
% Authors in alphabetical order.

\noindent
\mbox{H.\;Adhikary\href{https://orcid.org/0000-0002-5746-1268}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,14}},
\mbox{P.\;Adrich\href{https://orcid.org/0000-0002-7019-5451}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,16}},
\mbox{K.K.\;Allison\href{https://orcid.org/0000-0002-3494-9383}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,30}},
\mbox{N.\;Amin\href{https://orcid.org/0009-0004-7572-3817}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,5}},
\mbox{E.V.\;Andronov\href{https://orcid.org/0000-0003-0437-9292}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,26}},
\mbox{T.\;Anti\'ci\'c\href{https://orcid.org/0000-0002-6606-0191}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,3}},
\mbox{I.-C.\;Arsene\href{https://orcid.org/0000-0003-2316-9565}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,13}},
\mbox{M.\;Bajda\href{https://orcid.org/0009-0005-8859-1099}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,17}},
\mbox{Y.\;Balkova\href{https://orcid.org/0000-0002-6957-573X}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,19}},
\mbox{M.\;Baszczyk\href{https://orcid.org/0000-0002-2595-0104}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,18}},
\mbox{D.\;Battaglia\href{https://orcid.org/0000-0002-5283-0992}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,29}},
\mbox{A.\;Bazgir\href{https://orcid.org/0000-0003-0358-0576}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,14}},
\mbox{S.\;Bhosale\href{https://orcid.org/0000-0001-5709-4747}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,15}},
\mbox{M.\;Bielewicz\href{https://orcid.org/0000-0001-8267-4874}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,16}},
\mbox{A.\;Blondel\href{https://orcid.org/0000-0002-1597-8859}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,4}},
\mbox{M.\;Bogomilov\href{https://orcid.org/0000-0001-7738-2041}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,2}},
\mbox{Y.\;Bondar\href{https://orcid.org/0000-0003-2773-9668}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,14}},
\mbox{N.\;Bostan\href{https://orcid.org/0000-0002-1129-4345}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,29}},
\mbox{A.\;Brandin\textsuperscript{\,25}},
\mbox{W.\;Bryli\'nski\href{https://orcid.org/0000-0002-3457-6601}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,22}},
\mbox{J.\;Brzychczyk\href{https://orcid.org/0000-0001-5320-6748}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,17}},
\mbox{M.\;Buryakov\href{https://orcid.org/0009-0008-2394-4967}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,24}},
\mbox{A.F.\;Camino\textsuperscript{\,32}},
\mbox{P.\;Christakoglou\href{https://orcid.org/0000-0002-4325-0646}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,7}},
\mbox{M.\;\'Cirkovi\'c\href{https://orcid.org/0000-0002-4420-9688}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,27}},
\mbox{M.\;Csan\'ad\href{https://orcid.org/0000-0002-3154-6925}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,9}},
\mbox{J.\;Cybowska\href{https://orcid.org/0000-0003-2568-3664}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,22}},
\mbox{T.\;Czopowicz\href{https://orcid.org/0000-0003-1908-2977}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,14}},
\mbox{C.\;Dalmazzone\href{https://orcid.org/0000-0001-6945-5845}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,4}},
\mbox{N.\;Davis\href{https://orcid.org/0000-0003-3047-6854}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,15}},
\mbox{F.\;Diakonos\href{https://orcid.org/0000-0003-0142-9098}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,7}},
\mbox{A.\;Dmitriev\href{https://orcid.org/0000-0001-7853-0173}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,24}},
\mbox{P.~von\;Doetinchem\href{https://orcid.org/0000-0002-7801-3376}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,31}},
\mbox{W.\;Dominik\href{https://orcid.org/0000-0001-7444-9239}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,20}},
\mbox{P.\;Dorosz\href{https://orcid.org/0000-0002-8884-0981}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,18}},
\mbox{J.\;Dumarchez\href{https://orcid.org/0000-0002-9243-4425}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,4}},
\mbox{R.\;Engel\href{https://orcid.org/0000-0003-2924-8889}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,5}},
\mbox{G.A.\;Feofilov\href{https://orcid.org/0000-0003-3700-8623}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,26}},
\mbox{L.\;Fields\href{https://orcid.org/0000-0001-8281-3686}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,29}},
\mbox{Z.\;Fodor\href{https://orcid.org/0000-0003-2519-5687}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,8,21}},
\mbox{M.\;Friend\href{https://orcid.org/0000-0003-4660-4670}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,10}},
\mbox{M.\;Ga\'zdzicki\href{https://orcid.org/0000-0002-6114-8223}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,14,6}},
\mbox{O.\;Golosov\href{https://orcid.org/0000-0001-6562-2925}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,25}},
\mbox{V.\;Golovatyuk\href{https://orcid.org/0009-0006-5201-0990}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,24}},
\mbox{M.\;Golubeva\href{https://orcid.org/0009-0003-4756-2449}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,23}},
\mbox{K.\;Grebieszkow\href{https://orcid.org/0000-0002-6754-9554}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,22}},
\mbox{F.\;Guber\href{https://orcid.org/0000-0001-8790-3218}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,23}},
\mbox{S.N.\;Igolkin\textsuperscript{\,26}},
\mbox{S.\;Ilieva\href{https://orcid.org/0000-0001-9204-2563}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,2}},
\mbox{A.\;Ivashkin\href{https://orcid.org/0000-0003-4595-5866}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,23}},
\mbox{A.\;Izvestnyy\href{https://orcid.org/0009-0009-1305-7309}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,23}},
\mbox{K.\;Kadija\textsuperscript{\,3}},
\mbox{A.\;Kapoyannis\href{https://orcid.org/0000-0002-7732-8552}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,7}},
\mbox{N.\;Kargin\textsuperscript{\,25}},
\mbox{N.\;Karpushkin\href{https://orcid.org/0000-0001-5513-9331}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,23}},
\mbox{E.\;Kashirin\href{https://orcid.org/0000-0001-6062-7997}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,25}},
\mbox{M.\;Kie{\l}bowicz\href{https://orcid.org/0000-0002-4403-9201}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,15}},
\mbox{V.A.\;Kireyeu\href{https://orcid.org/0000-0002-5630-9264}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,24}},
\mbox{H.\;Kitagawa\textsuperscript{\,11}},
\mbox{R.\;Kolesnikov\href{https://orcid.org/0009-0006-4224-1058}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,24}},
\mbox{D.\;Kolev\href{https://orcid.org/0000-0002-9203-4739}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,2}},
\mbox{Y.\;Koshio\textsuperscript{\,11}},
\mbox{V.N.\;Kovalenko\href{https://orcid.org/0000-0001-6012-6615}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,26}},
\mbox{S.\;Kowalski\href{https://orcid.org/0000-0001-9888-4008}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,19}},
\mbox{B.\;Koz{\l}owski\href{https://orcid.org/0000-0001-8442-2320}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,22}},
\mbox{A.\;Krasnoperov\href{https://orcid.org/0000-0002-1425-2861}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,24}},
\mbox{W.\;Kucewicz\href{https://orcid.org/0000-0002-2073-711X}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,18}},
\mbox{M.\;Kuchowicz\href{https://orcid.org/0000-0003-3174-585X}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,21}},
\mbox{M.\;Kuich\href{https://orcid.org/0000-0002-6507-8699}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,20}},
\mbox{A.\;Kurepin\href{https://orcid.org/0000-0002-1851-4136}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,23}},
\mbox{A.\;L\'aszl\'o\href{https://orcid.org/0000-0003-2712-6968}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,8}},
\mbox{M.\;Lewicki\href{https://orcid.org/0000-0002-8972-3066}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,21}},
\mbox{G.\;Lykasov\href{https://orcid.org/0000-0002-1544-6959}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,24}},
\mbox{V.V.\;Lyubushkin\href{https://orcid.org/0000-0003-0136-233X}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,24}},
\mbox{M.\;Ma\'ckowiak-Paw{\l}owska\href{https://orcid.org/0000-0003-3954-6329}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,22}},
\mbox{Z.\;Majka\href{https://orcid.org/0000-0003-3064-6577}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,17}},
\mbox{A.\;Makhnev\href{https://orcid.org/0009-0002-9745-1897}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,23}},
\mbox{B.\;Maksiak\href{https://orcid.org/0000-0002-7950-2307}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,16}},
\mbox{A.I.\;Malakhov\href{https://orcid.org/0000-0001-8569-8409}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,24}},
\mbox{A.\;Marcinek\href{https://orcid.org/0000-0001-9922-743X}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,15}},
\mbox{A.D.\;Marino\href{https://orcid.org/0000-0002-1709-538X}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,30}},
\mbox{H.-J.\;Mathes\href{https://orcid.org/0000-0002-0680-040X}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,5}},
\mbox{T.\;Matulewicz\href{https://orcid.org/0000-0003-2098-1216}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,20}},
\mbox{V.\;Matveev\href{https://orcid.org/0000-0002-2745-5908}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,24}},
\mbox{G.L.\;Melkumov\href{https://orcid.org/0009-0004-2074-6755}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,24}},
\mbox{A.\;Merzlaya\href{https://orcid.org/0000-0002-6553-2783}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,13}},
\mbox{{\L}.\;Mik\href{https://orcid.org/0000-0003-2712-6861}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,18}},
\mbox{A.\;Morawiec\href{https://orcid.org/0009-0001-9845-4005}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,17}},
\mbox{S.\;Morozov\href{https://orcid.org/0000-0002-6748-7277}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,23}},
\mbox{Y.\;Nagai\href{https://orcid.org/0000-0002-1792-5005}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,9}},
\mbox{T.\;Nakadaira\href{https://orcid.org/0000-0003-4327-7598}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,10}},
\mbox{M.\;Naskr\k{e}t\href{https://orcid.org/0000-0002-5634-6639}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,21}},
\mbox{S.\;Nishimori\href{https://orcid.org/~0000-0002-1820-0938}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,10}},
\mbox{V.\;Ozvenchuk\href{https://orcid.org/0000-0002-7821-7109}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,15}},
\mbox{A.D.\;Panagiotou\textsuperscript{\,7}},
\mbox{O.\;Panova\href{https://orcid.org/0000-0001-5039-7788}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,14}},
\mbox{V.\;Paolone\href{https://orcid.org/0000-0003-2162-0957}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,32}},
\mbox{O.\;Petukhov\href{https://orcid.org/0000-0002-8872-8324}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,23}},
\mbox{I.\;Pidhurskyi\href{https://orcid.org/0000-0001-9916-9436}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,14,6}},
\mbox{R.\;P{\l}aneta\href{https://orcid.org/0000-0001-8007-8577}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,17}},
\mbox{P.\;Podlaski\href{https://orcid.org/0000-0002-0232-9841}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,20}},
\mbox{B.A.\;Popov\href{https://orcid.org/0000-0001-5416-9301}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,24,4}},
\mbox{B.\;P\'orfy\href{https://orcid.org/0000-0001-5724-9737}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,8,9}},
\mbox{M.\;Posiada{\l}a-Zezula\href{https://orcid.org/0000-0002-5154-5348}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,20}},
\mbox{D.S.\;Prokhorova\href{https://orcid.org/0000-0003-3726-9196}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,26}},
\mbox{D.\;Pszczel\href{https://orcid.org/0000-0002-4697-6688}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,16}},
\mbox{S.\;Pu{\l}awski\href{https://orcid.org/0000-0003-1982-2787}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,19}},
\mbox{J.\;Puzovi\'c\textsuperscript{\,27}\textsuperscript{\dag}},
\mbox{R.\;Renfordt\href{https://orcid.org/0000-0002-5633-104X}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,19}},
\mbox{L.\;Ren\href{https://orcid.org/0000-0003-1709-7673}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,30}},
\mbox{V.Z.\;Reyna~Ortiz\href{https://orcid.org/0000-0002-7026-8198}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,14}},
\mbox{D.\;R\"ohrich\textsuperscript{\,12}},
\mbox{E.\;Rondio\href{https://orcid.org/0000-0002-2607-4820}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,16}},
\mbox{M.\;Roth\href{https://orcid.org/0000-0003-1281-4477}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,5}},
\mbox{{\L}.\;Rozp{\l}ochowski\href{https://orcid.org/0000-0003-3680-6738}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,15}},
\mbox{B.T.\;Rumberger\href{https://orcid.org/0000-0002-4867-945X}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,30}},
\mbox{M.\;Rumyantsev\href{https://orcid.org/0000-0001-8233-2030}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,24}},
\mbox{A.\;Rustamov\href{https://orcid.org/0000-0001-8678-6400}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,1,6}},
\mbox{M.\;Rybczynski\href{https://orcid.org/0000-0002-3638-3766}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,14}},
\mbox{A.\;Rybicki\href{https://orcid.org/0000-0003-3076-0505}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,15}},
\mbox{K.\;Sakashita\href{https://orcid.org/0000-0003-2602-7837}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,10}},
\mbox{K.\;Schmidt\href{https://orcid.org/0000-0002-0903-5790}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,19}},
\mbox{A.Yu.\;Seryakov\href{https://orcid.org/0000-0002-5759-5485}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,26}},
\mbox{P.\;Seyboth\href{https://orcid.org/0000-0002-4821-6105}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,14}},
\mbox{U.A.\;Shah\href{https://orcid.org/0000-0002-9315-1304}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,14}},
\mbox{Y.\;Shiraishi\textsuperscript{\,11}},
\mbox{A.\;Shukla\href{https://orcid.org/0000-0003-3839-7229}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,31}},
\mbox{M.\;S{\l}odkowski\href{https://orcid.org/0000-0003-0463-2753}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,22}},
\mbox{P.\;Staszel\href{https://orcid.org/0000-0003-4002-1626}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,17}},
\mbox{G.\;Stefanek\href{https://orcid.org/0000-0001-6656-9177}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,14}},
\mbox{J.\;Stepaniak\href{https://orcid.org/0000-0003-2064-9870}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,16}},
\mbox{M.\;Strikhanov\textsuperscript{\,25}},
\mbox{H.\;Str\"obele\textsuperscript{\,6}},
\mbox{T.\;\v{S}u\v{s}a\href{https://orcid.org/0000-0001-7430-2552}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,3}},
\mbox{L.\;Swiderski\href{https://orcid.org/0000-0001-5857-2085}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,16}},
\mbox{J.\;Szewi\'nski\href{https://orcid.org/0000-0003-2981-9303}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,16}},
\mbox{R.\;Szukiewicz\href{https://orcid.org/0000-0002-1291-4040}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,21}},
\mbox{A.\;Taranenko\href{https://orcid.org/0000-0003-1737-4474}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,25}},
\mbox{A.\;Tefelska\href{https://orcid.org/0000-0002-6069-4273}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,22}},
\mbox{D.\;Tefelski\href{https://orcid.org/0000-0003-0802-2290}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,22}},
\mbox{V.\;Tereshchenko\textsuperscript{\,24}},
\mbox{A.\;Toia\href{https://orcid.org/0000-0001-9567-3360}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,6}},
\mbox{R.\;Tsenov\href{https://orcid.org/0000-0002-1330-8640}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,2}},
\mbox{L.\;Turko\href{https://orcid.org/0000-0002-5474-8650}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,21}},
\mbox{T.S.\;Tveter\href{https://orcid.org/0009-0003-7140-8644}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,13}},
\mbox{M.\;Unger\href{https://orcid.org/0000-0002-7651-0272~}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,5}},
\mbox{M.\;Urbaniak\href{https://orcid.org/0000-0002-9768-030X}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,19}},
\mbox{F.F.\;Valiev\href{https://orcid.org/0000-0001-5130-5603}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,26}},
\mbox{M.\;Vassiliou\textsuperscript{\,7}},
\mbox{D.\;Veberi\v{c}\href{https://orcid.org/0000-0003-2683-1526}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,5}},
\mbox{V.V.\;Vechernin\href{https://orcid.org/0000-0003-1458-8055}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,26}},
\mbox{V.\;Volkov\href{https://orcid.org/0000-0002-4785-7517}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,23}},
\mbox{A.\;Wickremasinghe\href{https://orcid.org/0000-0002-5325-0455}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,28}},
\mbox{K.\;W\'ojcik\href{https://orcid.org/0000-0002-8315-9281}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,19}},
\mbox{O.\;Wyszy\'nski\href{https://orcid.org/0000-0002-6652-0450}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,14}},
\mbox{A.\;Zaitsev\href{https://orcid.org/0000-0003-4711-9925}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,24}},
\mbox{E.D.\;Zimmerman\href{https://orcid.org/0000-0002-6394-6659}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,30}},
\mbox{A.\;Zviagina\href{https://orcid.org/0009-0007-5211-6493}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,26}}, and
\mbox{R.\;Zwaska\href{https://orcid.org/0000-0002-4889-5988}{\includegraphics[height=1.7ex]{figures/orcid-logo.png}}\textsuperscript{\,28}}
\\\rule{2cm}{.5pt}\\[-.5ex]\textit{\textsuperscript{\dag} \footnotesize deceased}


==> include/na61Institutions.tex <==
% based on XML DB with time Fri Apr 28 12:49:46 2023
% Institutes in alphabetical order.

\noindent
\textsuperscript{1}~National Nuclear Research Center, Baku, Azerbaijan\\
\textsuperscript{2}~Faculty of Physics, University of Sofia, Sofia, Bulgaria\\
\textsuperscript{3}~Ru{\dj}er Bo\v{s}kovi\'c Institute, Zagreb, Croatia\\
\textsuperscript{4}~LPNHE, University of Paris VI and VII, Paris, France\\
\textsuperscript{5}~Karlsruhe Institute of Technology, Karlsruhe, Germany\\
\textsuperscript{6}~University of Frankfurt, Frankfurt, Germany\\
\textsuperscript{7}~University of Athens, Athens, Greece\\
\textsuperscript{8}~Wigner Research Centre for Physics, Budapest, Hungary\\
\textsuperscript{9}~E\"otv\"os Lor\'and University, Budapest, Hungary\\
\textsuperscript{10}~Institute for Particle and Nuclear Studies, Tsukuba, Japan\\
\textsuperscript{11}~Okayama University, Japan\\
\textsuperscript{12}~University of Bergen, Bergen, Norway\\
\textsuperscript{13}~University of Oslo, Oslo, Norway\\
\textsuperscript{14}~Jan Kochanowski University, Kielce, Poland\\
\textsuperscript{15}~Institute of Nuclear Physics, Polish Academy of Sciences, Cracow, Poland\\
\textsuperscript{16}~National Centre for Nuclear Research, Warsaw, Poland\\
\textsuperscript{17}~Jagiellonian University, Cracow, Poland\\
\textsuperscript{18}~AGH - University of Science and Technology, Cracow, Poland\\
\textsuperscript{19}~University of Silesia, Katowice, Poland\\
\textsuperscript{20}~University of Warsaw, Warsaw, Poland\\
\textsuperscript{21}~University of Wroc{\l}aw,  Wroc{\l}aw, Poland\\
\textsuperscript{22}~Warsaw University of Technology, Warsaw, Poland\\
\textsuperscript{23}~Institute for Nuclear Research, Moscow, Russia\\
\textsuperscript{24}~Joint Institute for Nuclear Research, Dubna, Russia\\
\textsuperscript{25}~National Research Nuclear University (Moscow Engineering Physics Institute), Moscow, Russia\\
\textsuperscript{26}~St. Petersburg State University, St. Petersburg, Russia\\
\textsuperscript{27}~University of Belgrade, Belgrade, Serbia\\
\textsuperscript{28}~Fermilab, Batavia, USA\\
\textsuperscript{29}~University of Notre Dame, Notre Dame, USA\\
\textsuperscript{30}~University of Colorado, Boulder, USA\\
\textsuperscript{31}~University of Hawaii at Manoa, Honolulu, USA\\
\textsuperscript{32}~University of Pittsburgh, Pittsburgh, USA\\

